Learning to Learn in Interactive Constraint Acquisition

Constraint Programming (CP) has been successfully used to model and solve complex combinatorial problems. However, modeling is often not trivial and requires expertise, which is a bottleneck to wider adoption. In Constraint Acquisition (CA), the goal is to assist the user by automatically learning the model. In (inter)active CA, this is done by interactively posting queries to the user, e.g., asking whether a partial solution satisfies their (unspecified) constraints or not. While interac tive CA methods learn the constraints, the learning is related to symbolic concept learning, as the goal is to learn an exact representation. However, a large number of queries is still required to learn the model, which is a major limitation. In this paper, we aim to alleviate this limitation by tightening the connection of CA and Machine Learning (ML), by, for the first time in interactive CA, exploiting statistical ML methods. We propose to use probabilistic classification models to guide interactive CA to generate more promising queries. We discuss how to train classifiers to predict whether a candidate expression from the bias is a constraint of the problem or not, using both relation-based and scope-based features. We then show how the predictions can be used in all layers of interactive CA: the query generation, the scope finding, and the lowest-level constraint finding. We experimentally evaluate our proposed methods using different classifiers and show that our methods greatly outperform the state of the art, decreasing the number of queries needed to converge by up to 72%.

==> findscope_backup.tex <==
We now show why the current \textsc{FindScope}-based functions cannot be (efficiently) guided using the calculated probabilities for constraints, and we propose a new (simpler) function,
namely \textsc{G-FindScope}.

% Story:
% 1. Existing FindScope functions cannot be guided.
% 1.1 Briefly how they work
% 1.2 What is the problem to solve in each step
% 1.3 Findscope functions from the literature do this manually, with a recursive function -> logarithmic number of steps
% 1.4 We propose a simpler findscope function, following the above logic. In each step an optimization problem has to be solved, deciding the variables to keep. 
% 1.5  How to achieve same performance as existing findscope -> 


%%%%%% How to achieve same performance NOTES:
% Currently it is log|Y| for each variable ins the scope S!!!!!
% So it is |S|log|Y|		scope found minimal -> minimal |S|
% in our case, if we go scopes(B_Y') ~ scopes(B_Y)  / 2, then we care about the size of scopes(B), complexity = log |scopes(B)|, scopes(B) = |Y|^|S|

The functions used in the literature~\cite{bessiere2013constraint,tsouros2020efficient,bessiere2023learning} to find the scope of violated constraints after a negative answer from the user (line 8 of \cref{alg:general}) work in a similar way. They recursively map the problem of finding a constraint to a simpler problem by removing entire blocks of variables from the query and asking partial queries to the user. If after the removal of some variables, the answer of the user to the partial query posted changes to ``yes'', then the removed block contains at least one variable from the scope of a violated constraint. So, then {\em FindScope} focuses on this block, adding some variable assignments back to the example. When, after repeating this procedure, the size of the considered block becomes 1 (i.e. the block contains a single variable), this variable is found to be in the scope of a violated constraint we seek. The main differences between existing functions are regarding their mechanisms to avoid posting redundant queries to the user, and having some recursive calls that do not post a query. {\em FindScope} achieves a logarithmic complexity in terms of the number of queries posted to the user by splitting the variables approximately in half in each step. 

In practice, the problem we have to solve in each step is to find a set of variables $Y^{\prime} \subset Y$, with Y being the previously considered set of variables. Then, $e_{Y^{\prime}}$ is posted to the user, and depending on the answer we can update $B$ and decide in which part of the problem to focus on next. Existing {\em FindScope} functions manually choose $Y^{\prime} \subset Y$, by splitting $Y$ in half and using information from previously used sets of variables, given as parameters in each recursive call. The advantage of this approach is that a logarithmic number of steps is achieved. However, no information for the constraints from $B$ violated is used, neither any way of automated guiding can be directly utilized. The variables to remove, or keep, in the assignment are usually random~\cite{bessiere2023learning}. 

In this paper, we propose a simpler, non-recursive function to find the scope of violated constraints. We simplify the idea described in the previous paragraph and formulate the problem of finding the set of variables $Y^{\prime}$ to focus on as a CSP.
We observe that in each step, in order to avoid posting redundant queries to the user, we need to

\begin{equation}
\label{eq:guidefs}
\begin{aligned}
\text{find } Y^{\prime} \text{ s.t. } Y^{\prime} \subset Y \land 0 <  \kappa_B(e_{Y^{\prime}}) < \kappa_B(e_Y).
\end{aligned}
\end{equation}

In order to formulate the above as a CSP, we need to have a boolean variable $v_i$ for each variable $x_i \in Y$, representing the decision to include $x_i$ in $Y^{\prime}$ or not, i.e. $v_i = x_i \in Y^{\prime}$. The constraints to satisfy are: $Y^{\prime} \subset Y \land \kappa_B(e_{Y^{\prime}}) < \kappa_B(e_Y)$. By using this formalism in each step, we can now simplify the process. The proposed function, namely \textsc{G-FindScope}, is shown in \cref{alg:findscope}.

\hide{
\begin{enumerate}

\item $Y^{\prime} \subset Y$: this can be modeled with the constraint $\sum \llbracket v_i \rbracket < |Y|$

\item  $\kappa_B(e_{Y^{\prime}})  < \kappa_B(e_Y)$: this can be modeled as follows. Create a boolean variable for each constraint in $\kappa_B(e_Y)$ ... % too involved, no need to do that

\end{enumerate}
}


% New FindScope pseudocode -------------------------------------------------

\begin{algorithm}[t]
\caption{G-FindScope: Proposed Guided FindScope}\label{alg:findscope}
\begin{algorithmic}[1]

\Require $e$, $Y$, $B$
\Ensure $Scope$

\While {$\mid scopes(\kappa_B(e_Y))\mid$ $> 1$}

	\State $\text{find } Y^{\prime} \text{ s.t. }Y^{\prime} \subset Y \land 0 < |\kappa_B(e_{Y^{\prime}})| < |\kappa_B(e_Y)|$
  
        \If{$ASK(e_{Y^{\prime}})$ = True}    % \Comment{Post $e_{Y^{\prime}}$ to the user to classify it}
            \State $B \leftarrow B \setminus \kappa_B(e_{Y^{\prime}})$
        \Else
            \State $Y \leftarrow Y^{\prime}$
        \EndIf

\EndWhile

\State \Return $var(\kappa_B(e_Y))$


\end{algorithmic}
\end{algorithm}

% New FindScope pseudocode ------------------------------------------

\textsc{G-FindScope} takes as input the example $e$ in which we want to find the scope of a violated constraint, the set of assigned variables $Y$, and the bias $B$. It returns the a set of variables, which is the scope found. The main loop of the function starts at line ... In each step, the problem described previously is solved, in order to find the subset of variables $Y^{\prime}$ that will be considered in the next partial query. Then $e_{Y^{\prime}}$ is posted as a partial query to the user. If the answer is positive, then the candidate constraints violated by $e_{Y^{\prime}}$ are removed from $B$, so we can focus on different candidates in the next iteration. In case the answer is negative, then we know that (at least) one of the violated candidates is a constraint we need to learn, and thus we focus on them from now on, by replacing $Y$ by $Y^{\prime}$. In each iteration, the set of candidates considered is reduced as either constraints are removed from $B$ due to a positive answer, or the set of variables is reduced and thus also the candidates participating in the variables considered. The loop breaks when all the violated candidates in $B[Y]$ have the same scope. Hence, this scope is returned.

As the problem is now formulated as a CSP, it can also be converted to a COP, by including an objective function. The performance of \textsc{G-FindScope} will be directly affected by the objective function used in this step. Without using an objective function, the worst-case complexity in terms of the number of queries posted, which is equal to the number of iterations, is 

%\subsection{Analysis}

Let us now prove the correctness of \textsc{G-FindScope}.

%In this section, we first prove the correctness of \textsc{G-FindScope}. Next, we analyze its complexity in terms of the number of queries. We first give a complexity analysis when the function is used without an objective function, and then we show that by using a specific objective we can have similar complexity with the \textsc{FindScope} functions from the literature, thus achieving good results even when we cannot use any specialized objective to guide this procedure.
\dt{I wanted also to have complexity proofs for 2 cases (no objective + objective similar to normal FS), but correctness proof is huge so the others maybe will go to appendix (or just ignored them)}
% soundness:  var(B) is the scope of a violated constraint 
% reaching this line, we can only have the scope of 1 violated constraint in B. Thus, the set returned constraints the scope of a violated constraint. Now we have to prove that if a c \in C_T exists in \kappa_B(e_Y) in the beginning, it will never get removed and thus it will be the scope returned.
%
% completeness and termination: if there exists one or more violated constraints, a scope will be found.
% Prove that we reach return line -> prove that in each loop, scopes(\kappa_B(e_Y)) is reduced (and it will reach 1)

\begin{thm} 
\label{correctness_gfs}
Given a bias $B$, with an unknown target network $C_T$ being representable by $B$, a set of variables $Y$ and an example $e$ s.t. $\kappa_B(e_Y) \neq \emptyset$, \textsc{G-FindScope} is correct, i.e. it will return the scope of a constraint $c \in \kappa_{C_T}(e_Y)$.
\end{thm}

\begin{proof} (sketch)
In order to prove correctness, we will first prove soundness, i.e. that the set of variables returned at line 7 is always the scope of a constraint $c \in \kappa_{C_T}(e_Y)$, and then we will prove completeness and termination together, i.e. that \textsc{G-FindScope} always reaches line 7 to return a desired scope, if one exists.

(soundness) We will now prove that, if the function reaches line 7, then $var(\kappa_B(e_Y))$ is always the scope of a constraint $c \in \kappa_{C_T}(e_Y)$, assuming one exists. First, notice that when the function reaches line 7, then we know that $scopes(\kappa_B(e_Y)) \leq 1$ (from the condition at line 1). %, otherwise we would still be inside the loop of lines 1-6. 
Inside this loop, we can never end up in $scopes(\kappa_B(e_Y)) = \emptyset$ and
%$scopes(\kappa_B(e_Y)$ is always reduced either by removing constraints from $B$ at line 4 or by reducing the set of variables $Y$ considered at line 6. Based on how the set of variables $Y^{\prime}$ is chosen at line 2, we can never have $scopes(\kappa_B(e_Y)) = \emptyset$. That is because 
\hide{
%\begin{center}
\begin{equation}
\begin{aligned}
|\kappa_B(e_{Y^{\prime}})| < |\kappa_B(e_Y)| \\ 
\xRightarrow[line 4]{B \leftarrow B \setminus \kappa_B(e_{Y^{\prime}})} \kappa_B(e_Y) \setminus \kappa_B(e_{Y^{\prime}}) \neq \emptyset \\
\implies scopes(\kappa_B(e_Y)) \neq \emptyset
\end{aligned}
\end{equation}
%\end{center}
 and 
\begin{equation}
\begin{aligned}
0 < |\kappa_B(e_{Y^{\prime}})| \xRightarrow[line 6]{Y \leftarrow Y^{\prime}} \kappa_B(e_Y)  \neq \emptyset \\
\implies scopes(\kappa_B(e_Y)) \neq \emptyset
\end{aligned}
\end{equation}
}
%Thus, in line 7 we always have $|scopes(\kappa_B(e_Y))| = 1$. Let us now prove that this 
it will always contain the scope of a violated constraint of the problem, assuming one exists in the given example $e_Y$, i.e. $\exists c \in \kappa_B(e_Y)) \cap C_T$, as

\begin{equation}
\begin{gathered}
ASK(e_{Y^{\prime}}) = True \implies \nexists c \in \kappa_B(e_{Y^{\prime}})) \cap C_T \\ \xRightarrow[\text{line 4}]{\exists c \in \kappa_B(e_Y)) \cap C_T} \exists c \in \kappa_B(e_Y) \setminus \kappa_B(e_{Y^{\prime}}) 
\end{gathered}
\end{equation}

and

\begin{equation}
\begin{gathered}
ASK(e_{Y^{\prime}}) = False \implies \exists c \in \kappa_B(e_{Y^{\prime}})) \cap C_T \\ \xRightarrow[\text{line 6}]{Y \leftarrow Y^{\prime}} \exists c \in \kappa_B(e_Y) 
\end{gathered}
\end{equation}

As a result, after both lines 4 and 6, depending on the answer of the user, $\exists c \in \kappa_B(e_Y)$, and $\kappa_B(e_Y)$ does not change in any other part of the function. As a result, if line 7 is reached, $var(\kappa_B(e_Y))$ is always the scope of a constraint $c \in \kappa_{C_T}(e_Y)$.

%\exists c \in \kappa_B(e_Y)) \cap C_T$, which means that $var(\kappa_B(e_Y)) = var(c)$

(completeness)
Let us now prove completeness and termination together, i.e. that \textsc{G-FindScope} always reaches line 7 to return a desired scope, if one exists. Note that, as $e_{Y^{\prime}}$ is a projection of $e_Y$ in $Y^{\prime} \subset Y$, we know that 

\begin{equation}
\label{eq:subscopes}
\begin{gathered}
c \in \kappa_B(e_{Y^{\prime}}) \land var(c) = S \implies c \in \kappa_B(e_Y), \forall S \subset Y^{\prime}
\end{gathered}
\end{equation}

We will now prove that in each iteration of the loop at lines 1-6, the set $scopes(\kappa_B(e_Y))$ always reduces, and thus the condition at line 1 will finally get false. We use the subscripts $i$ and $i-1$ to denote the sets in iterations $i$ and $i-1$.

\begin{equation}
\begin{gathered}
0 < |\kappa_B(e_{Y^{\prime}})|  \\ 
\xRightarrow[\text{line 4}]{B \leftarrow B \setminus \kappa_B(e_{Y^{\prime}})} |\kappa_B(e_Y) \setminus \kappa_B(e_{Y^{\prime}})| < |\kappa_B(e_Y)| \\
\xRightarrow[]{Eq. (\ref{eq:subscopes})}  |scopes(\kappa_B(e_Y)\setminus \kappa_B(e_{Y^{\prime}}))| < |scopes(\kappa_B(e_Y))|
\end{gathered}
\end{equation}
%\end{center}
 and 
\begin{equation}
\begin{gathered}
|\kappa_B(e_{Y^{\prime}})| < |\kappa_B(e_Y)| \xRightarrow[\text{line 6}]{Y \leftarrow Y^{\prime}} |\kappa_B(e_Y)_i| < |\kappa_B(e_Y)_{i-1}| \\
\xRightarrow[]{Eq. (\ref{eq:subscopes})}  |scopes(\kappa_B(e_Y)_i)| < |scopes(\kappa_B(e_Y))_{i-1}|
\end{gathered}
\end{equation}
\end{proof}

% Theorem for correctness (soundness and completeness and termination).

%Having proven the correctness of \textsc{G-FindScope}, let us now focus on its complexity in terms of the number of queries.

% proposition for worst-case complexity without objective function
% proposition for worst-case complexity with scopes(B_Y') ~ scopes(B_Y)  / 2 objective

